A Stability-Based Abstraction Framework for Reach-Avoid Control of Stochastic Dynamical Systems with Unknown Noise Distributions

Finite-state abstractions are widely studied for the automated synthesis of correct-by-construction controllers for stochastic dynamical systems. However, existing abstraction methods often lead to prohibitively large finite-state models. To address this issue, we propose a novel abstraction scheme for stochastic linear systems that exploits the system's stability to obtain significantly smaller abstract models. As a unique feature, we first stabilize the open-loop dynamics using a linear feedback gain. We then use a model-based approach to abstract a known part of the stabilized dynamics while using a data-driven method to account for the stochastic uncertainty. We formalize abstractions as Markov decision processes (MDPs) with intervals of transition probabilities. By stabilizing the dynamics, we can further constrain the control input modeled in the abstraction, which leads to smaller abstract models while retaining the correctness of controllers. Moreover, when the stabilizing feedback controller is aligned with the property of interest, then a good trade-off is achieved between the reduction in the abstraction size and the performance loss. The experiments show that our approach can reduce the size of the graph of abstractions by up to 90% with negligible performance loss.

==> ECC-reviews-March2024.tex <==
#Reviewer6
- I could not find a way by which the authors manage to do the polyhedral partition of the state space. As far as I know, finding a polyhedral partition is extremely difficult for higher order state-space. I recommend that this point is carefully taken into consider in the final version of the paper. 

#Reviewer8
- I do not understand the stuff related to backward reachability. From what I see, it is just a way to discretize the action space. If I am not wrong, action a is enabled in s if the associated target point d_a is reachable from any point in the state-space region s, under the nominal (noise-free) dynamics. That way, you restrict how much you discretize the action space, as you consider only the actions a that take you to designated points d_a, but still it is a way to obtain a finite set of actions out from the original input space U. And, further, this is a 'biased' way of discretizing the action space, as the discretization is not done in some random uniform way, but in a way such that the actions take you to pre-specified points in the state space. Furthermore, I don't see how this is backward reachability. In the end, you still consider actions that take you from the current state s to some other state, and not vice-versa. In fact, even the feedback-refinement relation is defined in a forward-reachability way (via the transition kernel, which runs forward in time). Overall, more explanation is needed in that front (e.g., what is the advantage of doing that?).

- What are the true contributions of the paper? I see that the contribution is that the pant is stabilized before it is abstracted, and naturally all theoretical guarantees derived in previous papers follow in this case, as well. Thus, in my view, the contribution lies more in the numerical examples, where it is shown that if u stabilize
the plant, u might end up with a smaller abstraction. Nonetheless, as pointed out in the article as well, this is to be expected, up to a certain extent, if the stabilizing controller is aligned with the specification. Are there other contributions I might be missing?

- Including the set U' can be done even without stabilizing the plant beforehand. It just constrains the input space U even more, to U\cap U'. So, a more fair comparison would be to use U' even for the abstractions of the non-stabilized plant, and compare that to the abstractions for the stabilized plant.

- The scenario approach exposition is informal, and I think it gives rise to incorrect results. For example, it is not easy to see how by merely sampling the noise, one gets that the derived iMDP abstracts the system with some confidence. I suppose that the transition bounds are derived as the minimum and maximum frequency of reaching state s' from state s, among all sampled noise realizations. However, the probability that you sampled the precise noise realizations that give rise to the actual minimum and maximum probabilities is 0 (as the noise takes values in an uncountable set and you only take finite samples of it). So, the iMDP abstracts the actual system with confidence 0, because the transition bounds of the iMDP are not the actual minimum/maximum transition probabilities, with confidence 1. On the other hand, indeed, most likely, the fact that 'the specification satisfaction probability over the real system is lower bounded by the satisfaction probability over the iMDP' indeed has confidence 1-beta. Though, this is not the same as saying 'the iMDP abstracts the system with confidence 1-beta'. This needs careful consideration.

- The iMDP exposition is a bit informal, although I don't think it harms validity of the results. For example, in the maxmin problem, the min has to be considered among all _adversaries_ in the iMDP and not among all possible P' in P. That is because, especially for finite-horizon properties, optimal adversaries are time-varying. If u constraint your search in to be among P' in P, you essentially constrain your search over time-invariant adversaries. Nonetheless, conventional value-iteration over iMDPs does address time-varying adversaries, and this is what the authors use in the end, I guess.

- In eq(12), it has to be specified that it is "for all x in s". 

#Reviewer9


Reviewer10
1. The paper would benefit from additional experimental validation using real-world data or more complex system models to demonstrate the method's practical efficacy.

2. While the assumptions on system dynamics and noise properties are necessary for your approach, it would be valuable to discuss their implications in terms of the method's generalizability and limitations.

3. A detailed comparison with existing methods would enrich the paper, providing the reader with a clear understanding of the proposed method's advantages and potential trade-offs.

4. A more comprehensive discussion on the computational complexity and scalability of the proposed method would be beneficial, as it would offer insight into its applicability to large-scale systems.

5. The manuscript could also explore the robustness of the method against variations in system parameters and its sensitivity to noise characteristics.
